SEIGAN: Towards Compositional Image Generation by Simultaneously Learning to Segment, Enhance, and Inpaint

We present a novel approach to image manipulation and understanding by simultaneously learning to segment object masks, paste objects to another background image, and remove them from original images. For this purpose, we develop a novel generative model for compositional image generation, SEIGAN (Segment-Enhance-Inpaint Generative Adversarial Network), which learns these three operations together in an adversarial architecture with additional cycle consistency losses. To train, SEIGAN needs only bounding box supervision and does not require pairing or ground truth masks. SEIGAN produces better generated images (evaluated by human assessors) than other approaches and produces high-quality segmentation masks, improving over other adversarially trained approaches and getting closer to the results of fully supervised training.

==> coco_city.tex <==
\begin{table*}
\renewcommand{\arraystretch}{0.6}
\setlength{\tabcolsep}{1.0pt}
\label{fig:examples-array}
\begin{center}
\begin{tabular}{ccccccc}
\hline
    Method & $\x$ & $\y$ & $\z$ & $\hy$ & $\hx$ & $\m$  \\
\hline
    \rotatebox{90}{SEIGAN}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_real_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_real_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_fake_inserted.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_fake_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_fake_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/1e79c517_mask_one.png}
        \\
    \rotatebox{90}{SEIGAN}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_real_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_real_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_fake_inserted.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_fake_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_fake_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/286b558d_mask_one.png}
        \\
    \rotatebox{90}{SEIGAN}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_real_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_real_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_fake_inserted.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_fake_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_fake_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e06f7608_mask_one.png}
        \\
    \rotatebox{90}{SEIGAN}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_real_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_real_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_fake_inserted.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_fake_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_fake_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/e0883545_mask_one.png}
        \\
\hline
    \rotatebox{90}{NoCycle}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_real_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_real_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_fake_inserted.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_fake_B.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_fake_A.png}
        & \includegraphics[width=0.15\linewidth]{images/examples_array/0b81b288_mask_one.png}
        \\
\hline
\end{tabular}
\end{center}
\caption{Some samples of successful images and failures of our method and its variants.}
\end{table*}
